ArcSin: Adaptive ranged cosine Similarity injected noise for Language-Driven Visual Tasks

"A data scientist is tasked with developing a low-cost surgical VQA system for a 2-month workshop. Due to data sensitivity, she collects 50 hours of surgical video from a hospital, requiring two months for privacy approvals. Privacy restrictions prevent uploading data to platforms like ChatGPT, so she assembles one annotator and a medical expert to manually create QA pairs. This process takes three weeks and costs over $10,000. The trained model provides accurate responses within the limited data scope but lacks broader generalizability, completing the project in 3 months." To simplify the challenges presented in the scenario above. In this paper, we replace the image input with text for Vision-language training. Inspired by prior noise injection methods to reduce modality gaps, we introduce Adaptive ranged cosine Similarity injected noise (ArcSin). First, we introduce an innovative adaptive noise scale that effectively generates the textual elements with more variability while preserving the original text feature's integrity. Second, a similarity pool strategy is employed, expanding the domain generalization potential by broadening the overall noise scale. This dual strategy effectively broadens the scope of the original domain while safeguarding content integrity. Our empirical results demonstrate that these models closely rival those trained on images in terms of performance. Specifically, our method exhibits substantial improvements over the previous state-of-the-art, achieving gains of 1.9 and 1.1 CIDEr points in S-Cap and M-Cap, respectively. Additionally, we observe increases of 0.5 percentage points (pp), 1.4 pp, and 1.4 pp in accuracy for VQA, VQA-E, and VE, respectively, pushing the boundaries of what is achievable within the constraints of image-trained model benchmarks.

==> picture/Fig_bad_ex_sup.tex <==
\begin{figure*}[h]
\centering
\includegraphics[width=0.8\linewidth]{picture/bad_ex_sup.pdf}
\caption{\textbf{Supplementary failure cases in the Cap (S-Cap and M-Cap), VE, and VQA (VAQ and VQA-E) tasks by \method{} and CLOSE.}}
\label{sfig:bad_ex_sup}
\centering
\end{figure*}

==> picture/Fig_diff_styles_sup.tex <==
\begin{figure*}[h]
\centering
\includegraphics[width=0.8\linewidth]{picture/Samples_Different_Styles.pdf}
\caption{\textbf{Supplementary cross-style captioning cases.} Our \method{} model, trained on M-Cap, demonstrates its robust captioning ability on some different style images with distinct visual styles, randomly sourced from the web.}
\label{sfig:diffstyle}
\centering
\end{figure*}

==> picture/Fig_ex_sup.tex <==
\begin{figure*}[h]
\centering
\includegraphics[width=0.9\linewidth]{picture/ex_sup.pdf}
\caption{\textbf{Supplementary qualitative comparisons with state-of-the-art method CLOSE in the Cap (S-Cap and M-Cap), VE, VQA (VAQ and VQA-E) tasks.}}
\label{sfig:ex_sup}
\centering
\end{figure*}

==> picture/Fig_scale-sim.tex <==
\begin{figure}[h]
\centering
\includegraphics[width=\linewidth]{picture/scale-sim.pdf}
\caption{\textbf{Illustrating the trade-off between noise scale and feature fidelity, this graph compares the impact of various noise injection strategies on similarity retention.} From the COCO dataset~\cite{chen2015microsoft}, 20 image-text pairs were randomly sampled, and their features encoded using the CLIP-ViT B/32 model~\cite{Radford2021-CLIP}. The noise scale's average across different feature dimensions and instances is plotted on the horizontal axis, while the vertical axis measures the average similarity score. All methods exhibit a general trend where increased noise correlates with reduced similarity. Notably, CLOSE (orange) and \method{} without an Injection Pool (green) display similar trends of declining similarity. In contrast, \method{} with an Injection Pool (red) maintains higher similarity scores, indicating a robustness to noise across the measured range.}
\label{sfig:scale-sim}
\centering
\vspace{-2mm}
\end{figure}

==> picture/Fig_tsne.tex <==

\begin{figure*}[h]
\centering
\includegraphics[width=\linewidth]{picture/Fig_compare_Close_differentSIM_temporal.pdf}
\caption{\textbf{t-SNE~\cite{TSNE} visualization of noise-injected features from various methods.} For different cosine similarity-constrained noise injection, we analyzed 400 image-text pairs (shown as red-blue points). The image-text content variations are more densely grouped, which implies that the feature space is mainly influenced by the domain gap. Features enhanced by our \method{} (orange points) exhibit broader domain coverage at cosine similarities of 0.3 and 0.4, facilitating the acquisition of more generalizable features. In contrast, the CLOSE's noise-injected features (green points) show minimal deviation from the original text features, leading to limited augmentation effectiveness. At a reduced similarity threshold of 0.1, both methods reach closer to the image feature domain; however, this aggressive injection compromises performance, indicating that excessive noise can alter the content significantly.
}


\label{fig:visulize_tsne_features}
\centering
\end{figure*}

==> picture/fig_sup_surgical.tex <==
\begin{figure}[h!]
\centering
\includegraphics[width=\linewidth]{picture/Surgical_examples.pdf}
\caption{\textbf{Surgical VQA Cases.} Our \method{} is trained on synthetic descriptions and Q\&A pairs generated by ChatGPT, with inference performed on surgical images selected from Cholec80~\cite{twinanda2016endonet}.}
\label{sfig:surgical_examples}
\centering
\end{figure}

==> preamble.tex <==
%
% --- inline annotations
%
\newcommand{\red}[1]{{\color{red}#1}}
\newcommand{\todo}[1]{{\color{red}#1}}
\newcommand{\TODO}[1]{\textbf{\color{red}[TODO: #1]}}
% --- disable by uncommenting  
% \renewcommand{\TODO}[1]{}
% \renewcommand{\todo}[1]{#1}



==> table/Tab_unify_parameters.tex <==



\begin{table}[t]
\centering
\caption{\textbf{Comparison with the state-of-the-art method while adopting the consistent hyperparameter across different V\&L tasks.} We report the CIDEr ($\uparrow$) score for S-Cap and M-Cap, and the accuracy percentages ($\uparrow$) for VQA, E-VQA, and VE.}
\setlength{\tabcolsep}{6.6pt}
\renewcommand{\arraystretch}{1.2}
\resizebox{\linewidth}{!}
{
\begin{tabular}{cccccc} 
\toprule 
\hline
Method & S-Cap & M-Cap &VQA &VQA-E & VE \\
\cline{2-6}
%& C & C & Acc & Acc &Acc\\
\hline
CLOSE &80.5   & 95.3 & \textbf{59.6}  &62.9   & 74.6   \\
\method{} (Ours)&\textbf{90.8}   & \textbf{97.0} &\textbf{59.6}   &\textbf{63.7}   & \textbf{75.2}  \\
\midrule 
\bottomrule 
\end{tabular}
}


\label{table:unified_parameters}
\end{table}




